Free Lunch for Efficient Textual Commonsense Integration in Language Models

Recent years have witnessed the emergence of textual commonsense knowledge bases, aimed at providing more nuanced and context-rich knowledge. The integration of external commonsense into language models has been shown to be a key enabler in advancing the state-of-the-art for a wide range of NLP tasks. However, incorporating textual commonsense descriptions is computationally expensive, as compared to encoding conventional symbolic knowledge. In this paper, we propose a method to improve its efficiency without modifying the model. We group training samples with similar commonsense descriptions into a single batch, thus reusing the encoded description across multiple samples. One key observation is that the upper bound of batch partitioning can be reduced to the classic {\it graph k-cut problem}. Consequently, we propose a spectral clustering-based algorithm to solve this problem. Extensive experiments illustrate that the proposed batch partitioning approach effectively reduces the computational cost while preserving performance. The efficiency improvement is more pronounced on larger datasets and on devices with more memory capacity, attesting to its practical utility for large-scale applications.

==> fast_model.tex <==
\section{Integrate textual knowledge into language models}
In this section, we describe how to encode textual knowledge via a pre-trained language model and  incorporate the hidden states of that knowledge into the target textual representation. Our model TELM uses KnowBERT, a structured knowledge enpowered language model, as the backbone. We will briefly introduce KnowBERT first in Sec x. Then in Sec x we illustrate  how we modify KnowBERT so that TELM can incorporate textual knowledge and improve its efficiency. We will illustrate in Sec x how the model is fine-tuned for the downstream task without continue pre-training.

\subsection{Background: Integrating knowledge via KnowBERT}
KnowBERT is a typical knowledge integration model based on BERT. It focuses on entity knowledge from a knowledge graph. External entity knowledge is represented as entity embeddings and incorporated into the mention spans of the target text through the Attention mechanism. More specifically, each layer of KnowBERT is computed as follows.
\begin{enumerate}
\item (Mention-span representations) First, KnowBERT uses self-attentive span pooling~\cite{} to compute the hidden states of each span. 
\item (Entity linker) Then, based on the attention mechanism, it computes the score of each span to each entity. 
\item (Knowledge enhancement) The entity embedding of each span is computed by the weighted entity embeddings of each entity based on the scores. 
\item (Recontextualization) Finally, using the Transformer model, the new hidden state of words are computed by taking the original hidden state of word as query and the entity embeddings of spans as keys/values. The new hidden state is added to the original hidden state to get the final hidden state of each word in the layer.
\end{enumerate}

\subsection{Textual knowledge integration and efficiency optimization}
TELM works similarly with KnowBERT. Instead of incorporating static entity embeddings in KnowBERT, TELM incorporate dynamic encodings of the textual knowledge. We use a tunable language model to encode the textual knowledge, so that the encodings can be updated during fine-tuning. In addition, we also optimize some modules of KnowBERT to make TELM simpler and more efficient.

Each layer of the TELM model is an extension of the layer of KnowBERT. The $i$-th layer receives the hidden states $H^{(i-1)}$ of the previous layer, and computes the new hidden states $H^{(i)}$.

{\bf Verb-span representation} Similar to KnowBERT's mention-span representations, TELM uses the representation of each verb-span to interact with the knowledge base. For each verb-span, we directly use the hidden state of the first token from $H^{(i-1)}$ as its representation. For a sentence with $C$ verb spans, their hidden states are stacked into a matrix $S = \mathcal{R}^{C \times d}$.
Here, we do not apply an extra self-attention to $S$ as in KnowBERT to improve the model efficiency. %And we abandon the self-attentive span pooling to improve the efficiency. 

%Unlike the use of self-attentive span pooling in KnowBERT, to improve efficiency, we directly use the verb's hidden state in $H^{(i-1)}$. For a sentence with $C$ verbs, their hidden states are stacked into a matrix $S = \mathcal{R}^{C \times d}$.

{\bf Textual knowledge representation} Instead of static entity embeddings in KnowBert, each textual knowledge description is encoded via a pre-trained LM in TELM. The parameters of this LM is tunable. The LM for the textual knowledge and the LM for the target sentence have separate parameters. For a knowledge description $t_j$, we compute its knowledge embedding by:
\begin{equation}
e^{(i)}_j = LM^{(i)}(t_j)
\end{equation}
where $LM^{(i)}(t_j)$ denotes the hidden state in the $i$-th layer. %We use the text encoding of the same layer as TELM. %knowledge introduced for the $i$-th layer of TELM.

{\bf Knowledge linker} The textual knowledge linker is used to calculate the score of each verb span to its corresponding knowledge. For a verb span $v$, we calculate the scores as:
\begin{equation}
    \psi_{vj} = MLP(S_v \cdot e^{(i)}_{j})
\end{equation}

{\bf Knowledge enhancement} We use the attention mechanism to compute the knowledge embedding of each verb span based on $\psi_{vj}$:
\begin{equation}
    \tilde{e}_v = \sum_k \psi_{vj} e_{j}
\end{equation}

{\bf Recontextualization} The verb representations are updated with their textual knowledge embeddings. To improve efficiency, we replace KnowBERT's multi-head attention with a direct addition to these verbs:
\begin{equation}
    H^{(i)}_v = H^{(i-1)}_v + \tilde{e}_v
\end{equation}
The representation of the rest words will stay unchanged.

\subsection{Training}
We initialize the LMs for the target sentence and the textual knowledge separately via the pre-trained parameters. We randomly initialize the rest parameters in TELM, i.e., the parameters used to integrate hidden states of the textual knowledge via attention. Then, without continuing pre-training over unsupervised corpora, we directly fine-tune the model in the downstream task. All parameters, including these of the textual knowledge encoder, will be updated during training.
